Four families of maximal real algebraic hypersurfaces in $\mathbb{RP}^4$

In this paper, we present four families of maximal real algebraic hypersurfaces of even degree in $\mathbb{RP}^4$ constructed using O. Viro's combinatorial patchworking method. We compare the Euler characteristic of the real part and the signature of the complex part of double coverings of $\mathbb{CP}^4$ ramified over the complex part of the constructed real algebraic hypersurfaces. We prove that these invariants are not necessarily equal and can even be asymptotically different.

==> figures.tex <==
\appendix

\section{Figures}



\begin{center}
    \includegraphics[scale=1]{images/cycles-avril-susp.png}
    \begin{minipage}{16cm}
    \begin{it}
    \small{Fig. 2: In green, the intersection of the patchworked surface with the union of the stars of the essential parts of the axes of pairs from Sections \ref{11a}, \ref{susp20}, \ref{11b} (from left to right). The colors of the vertices represent their signs.}
    \end{it}
    \end{minipage}
\end{center}

\begin{center}
    \includegraphics[scale=0.4]{images/11d.png}
    \begin{minipage}{16cm}
    \begin{it}
    \small{Fig. 3: Four copies of $T_4$ are represented. We suppose that the vertices of the suspensions over these four copies are the same. On the left, the integer points in $T_4$ are endowed with a non-Harnack sign distribution. On the right, the sign distribution is a Harnack one. The colors of the vertices represent their sign. The intersection of the patchworked surface with the considered copies of $T_4$ appears in green. The red broken lines are axes corresponding to the description of Section \ref{11d}. Each blue broken line corresponds to a broken line named $C$ from Section \ref{11d}.}
    \end{it}
    \end{minipage}
\end{center}

\begin{center}
    \includegraphics[scale=0.4]{images/suspspecial.png}
    \begin{minipage}{16cm}
    \begin{it}
    \small{Fig. 4: Four copies of $T_4$ are represented. We suppose that the vertices of the suspensions over these four copies are the same. On the left, the integer points in $T_4$ are endowed with a non-Harnack sign distribution. On the right, the sign distribution is a Harnack one. The colors of the vertices represent their sign. The intersection of the patchworked surface with the considered copies of $T_4$ appears in green. The red broken lines are two segments from axes corresponding to the description of Section \ref{suspspecial} (the two other segments of such axis lie in the other four copies of $T_4$). Each blue broken line corresponds to a broken line named $C$ from Section \ref{suspspecial}.}
    \end{it}
    \end{minipage}
\end{center}

\begin{center}
    \includegraphics[scale=1]{images/cycles-avril-join.png}
    \begin{minipage}{16cm}
    \begin{it}
    \small{Fig. 5: In green, the intersection of the patchworked surface with the star of the essential segment of an axis from a pair described in \ref{join}. The colors of the vertices represent their signs.}
    \end{it}
    \end{minipage}
\end{center}

    \begin{center}
    \includegraphics[scale=0.7]{images/regular-wall-odd.png}
    \begin{minipage}{16cm}
    \begin{it}
    \small{Fig. 6: On the left and on the right, two adjacent copies of a cone over $T_3$ and of a join of $S_3$ and $S_2$ are represented. The colors of the integer points (blue or red) represent their sign. On the left, a cycle axis pair as described in Section \ref{wallregu}. The cycle is green, the axis is red. Neither the axis nor the cycle is contained in a single orthant. On the right, the pair after the axis modification explained in Section \ref{wallregu}. The axis is now contained in a single orthant.}
    \end{it}
    \end{minipage}
\end{center}
    \begin{center}
    \includegraphics[scale=0.7]{images/regular-wall-even.png}
    \begin{minipage}{16cm}
    \begin{it}
    \small{Fig. 7: On the left and on the right, two adjacent copies of a cone over $T_4$ and of a join of $S_4$ and $S_3$ are represented. The colors of the integer points (blue or red) represent their sign. On the left and on the right, a cycle-axis pair as described in Section \ref{wallregu}. Cycles are green, axes are red or blue. On the right, one extremity of the essential part of the axis is of the same parity as the extremities of $S_4$. On the left, the parities of both extremities of the essential part of the axis are different from the parity of the extremities of $S_4$.}
    \end{it}
    \end{minipage}
\end{center}

\begin{center}
    \includegraphics[scale=0.7]{images/special-wall.png}
    \begin{minipage}{16cm}
    \begin{it}
    \small{Fig. 8: Two adjacent copies of a cone over $T_4$ and of a join of $S_4$ and $S_3$ are represented, as well as the copy of another cone over $T_4$. The colors of the integer points (blue or red) represent their sign. A typical suspension pair cycle appears in green. The dual axis appears in blue. In this case, the sign distribution on $T_4$ is not a Harnack one, hence the axis can be chosen to be contained in a single orthant.}
    \end{it}
    \end{minipage}
\end{center}

\begin{center}
    \includegraphics[scale=0.4]{images/trick1.png}
    \begin{minipage}{16cm}
    \begin{it}
    \small{Fig. 9: Illustration of an axis (in yellow) corresponding to the last set of axes described in Section \ref{0001111222}. These axes pass through several orthants. The equations indicate the hyperplane or intersection of hyperplane in a copy of which the objects lie. The left hand side shows where the considered triangles are located. On the right hand side, the intersection of the patchworked $3$-manifold with the represented triangles appears in green. The blue (respectively red) dots represent vertices of cones over blue (respectively red) triangles. The white dots with red or blue contour are copies of extremities of the essential part of the axis.}
    \end{it}
    \end{minipage}
\end{center}

\begin{center}
    \includegraphics[scale=0.5]{images/wall-of-cone.png}
    \begin{minipage}{16cm}
    \begin{it}
    \small{Fig. 10: On the left, an illustration of a cycle as described in Section \ref{wallcone} that is contained in a single orthant. On the right, an illustration of a cycle as described in Section \ref{wallcone} that is not contained in a single orthant. The equations indicate the hyperplane or intersection of hyperplane in a copy of which the objects lie. The colors of the points represent their sign. The cycle partially appears in green. In both cases, the missing part of the cycle is the cone over the green circle lying in the blue triangle with vertex the green point.}
    \end{it}
    \end{minipage}
\end{center}

\begin{center}
    \includegraphics[scale=0.4]{images/trick2.png}
    \begin{minipage}{16cm}
    \begin{it}
    \small{Fig. 11: Illustration of an axis (in yellow) corresponding to the description of the last set of axes in Section \ref{wall2}. This axis pass through several orthants. The equations indicate the hyperplane or intersection of hyperplane in a symmetric copy of which the objects lie. The left hand side shows where the considered objects are located. On the right hand side, the intersection of the patchworked $3$-manifold with the represented triangles appears in green. The blue (respectively red) points represent vertices of cones over blue (respectively red) triangles. A copy of any integer point that was named in Section \ref{wall2} bears the name of this point.}
    \end{it}
    \end{minipage}
\end{center}

\begin{center}
    \includegraphics[scale=0.35]{images/triangulation-z0.png}\\
    \begin{minipage}{16cm}
    \begin{it}
    \small{Fig. 12:  The important segments in the $((5,0,0),(0,3,0))$-SD triangulation of $\Delta_9^3 \bigcap \{ z=0 \}$, following the description in Section \ref{trimodif}}
    \end{it}
    \end{minipage}
\end{center}

\begin{center}
    \includegraphics[scale=0.285]{images/triangulationmodif.png}\\
    \begin{minipage}{16cm}
    \begin{it}
    \small{Fig. 13: Subdividing $C$ following step by the description in Section \ref{trimodif}. On the picture in the bottom right corner, $C$ is split along $C_1$ for readability purposes.}
    \end{it}
    \end{minipage}
\end{center}

\begin{center}
    \includegraphics[scale=0.8]{images/gudkovcurve.png}\\
    \begin{minipage}{16cm}
    \begin{it}
    \small{Fig. 14:  The curve obtained by restricting the $((5,0,0),(0,3,0))$-SD datum on $\Delta_9^3$ (here, $k=4$) to the triangle with vertices (0, 0, 0), (7, 0, 0), (0, 6, 0). White dots represent integer points bearing
    the sign $-$, black dots represent integer points bearing the sign $+$. Some important edges of the triangulation are drawn in black. The curve is sketched in red.}
    \end{it}
    \end{minipage}
\end{center}

\begin{center}
    \includegraphics[scale=0.7]{images/modifasympto.png}\\
    \begin{minipage}{16cm}
    \begin{it}
    \small{Fig. 15: The curve associated to a certain $L$-AD datum restricted to a triangle labeled $1$ whose edges are of lattice length $8$. Here, we have $a_8=(7,0,1,m-8)$, $b_8=(1,0,7,m-8)$, $c_8=(2,3,3,m-8)$. We have taken a copy in the plane $\mathbb{R}^2$ of the triangle. Black dots represent integer points bearing the sign $+$. White dots represent integer points bearing the sign $-$. The curve appears in red. It is a maximal curve, as there are $22$ connected components.}
    \end{it}
    \end{minipage}
\end{center}

%\begin{center}
%    \includegraphics[scale=1.25]{images/quantities.png}\\
%    \begin{minipage}{16cm}
%    \begin{it}
%    \label{quantities}
%    \small{Fig. 16: Two primitive triangulations of the triangle with vertices $(0,0)$, $(4,0)$, $(0,4)$.}
%    \end{it}
%    \end{minipage}
%\end{center}
